Achieving Near Instance-Optimality and Minimax-Optimality in Stochastic and Adversarial Linear Bandits Simultaneously

In this work, we develop linear bandit algorithms that automatically adapt to different environments. By plugging a novel loss estimator into the optimization problem that characterizes the instance-optimal strategy, our first algorithm not only achieves nearly instance-optimal regret in stochastic environments, but also works in corrupted environments with additional regret being the amount of corruption, while the state-of-the-art (Li et al., 2019) achieves neither instance-optimality nor the optimal dependence on the corruption amount. Moreover, by equipping this algorithm with an adversarial component and carefully-designed testings, our second algorithm additionally enjoys minimax-optimal regret in completely adversarial environments, which is the first of this kind to our knowledge. Finally, all our guarantees hold with high probability, while existing instance-optimal guarantees only hold in expectation.

==> lower_bound.tex <==
\section{Lower Bounds}\label{app: lower bound}
In this section, we focus on regret lower bounds of consistent policies in the stochastic setting.
Given loss vector $\ell$ and hidden action set $\calX$ with a unique optimal arm $x^*$. 
Then for any consistent algorithm, the expected pseudo-regret $\pReg(T)$ satisfies:
\begin{align*}
    \liminf_{T\to\infty}\frac{\pReg(T)}{\log T}\ge c(\calX,\ell),
\end{align*}
where $c(\calX,\ell)$ is the solution to the following optimization problem:
\begin{align*}
    &\inf_{N\in[0, \infty)^\calX} \sum_{x\in \calX\backslash\{x^*\}}N_x\Delta_x \\
    \text{subject to\ \ } & \|x\|^2_{H^{-1}(N)}\leq \frac{\Delta_x^2}{2},\quad\forall {x\in \calX\backslash\{x^*\}}
\end{align*}
where $H(N)=\sum_{x\in\calX}N_x xx^\top $. 

On the other hand, previous works showed that there exist algorithms matching this asymptotic bound (see, for example, the algorithm in \citep{lattimore2017end}), that is, for all $\ell\in\mathbb{R}^d$, the algorithms are asymptotically optimal in the sense that they guarantee
\begin{align*}
    \liminf_{T\to\infty}\frac{\pReg(T)}{\log T}\le c(\calX,\ell).
\end{align*}
However, in the following we show that these algorithms are vulnerable to adversarial environments. 
More specifically, we show no algorithm with $\order(\log T)$ pseudo-regret in the stochastic linear bandits can guarantee a sublinear regret bound against an oblivious adversary with high probability. 
The statement comes directly from the following theorem:
\begin{theorem}\label{thm:hp lower bound}
    If an algorithm guarantees a pseudo-regret bound of  
    \begin{align*}
        c_{\Reg}\cdot c(\calX,\ell)\frac{1-\gamma}{\log \frac{4}{\Delta_{\min}}}(\log T)^2   
    \end{align*} for constant $c_{\Reg}=\frac{\gamma}{64}$ 
    in the stochastic environment for all sufficiently large $T$, then for all $\gamma\in(0,1)$, it cannot guarantee a $O(T^\gamma \Delta_{\min})$ high-probability regret bound against an oblivious adversary. 
\end{theorem}
The proof is deferred to Appendix and the idea is similar to Theorem 2 in \citep{auer2016algorithm}.
\pref{thm:hp lower bound} inspires us to design an algorithm that is nearly (asymptotically) optimal and is robust to adversaries and corruptions with high probability, which is presented in the next section. 

The asymptotic lower bound may be vacuous when $T$ is finite. Here we provide another lower bound when $T$ is finite.
\begin{theorem}
    Let $\calA$ be an algorithm with nearly-optimal pseudo-regret bound in any instance that has $T$ interactions. Then in a problem instance with $\Delta_{\min}>0$ which satisfies
    \begin{align*}
        \frac{T^{1-2\epsilon}}{\ln T}\geq \frac{64U^2d^2}{\Delta_{\min}^2}
    \end{align*}
    for some $\epsilon>0$, 
    the pseudo-regret is lower bounded by the optimal value of the optimization below: 
    \begin{align*}
        &\min_{N_x\geq 0} N_x \Delta_x \\
        \text{subject to}\ \ & \|x\|_{H(N)^{-1}}^2 \leq \frac{4}{\epsilon \ln T}\Delta_x^2 + \frac{16}{7T},\\
        & \sum_{x}N_x = T. \left(= \frac{t}{2048}\right)
   \end{align*}
   where $H(N)\triangleq \sum_{x}N_x xx^\top$. 
\end{theorem}
